ROSAR: An Adversarial Re-Training Framework for Robust Side-Scan Sonar Object Detection

This paper introduces ROSAR, a novel framework enhancing the robustness of deep learning object detection models tailored for side-scan sonar (SSS) images, generated by autonomous underwater vehicles using sonar sensors. By extending our prior work on knowledge distillation (KD), this framework integrates KD with adversarial retraining to address the dual challenges of model efficiency and robustness against SSS noises. We introduce three novel, publicly available SSS datasets, capturing different sonar setups and noise conditions. We propose and formalize two SSS safety properties and utilize them to generate adversarial datasets for retraining. Through a comparative analysis of projected gradient descent (PGD) and patch-based adversarial attacks, ROSAR demonstrates significant improvements in model robustness and detection accuracy under SSS-specific conditions, enhancing the model's robustness by up to 1.85%. ROSAR is available at https://github.com/remaro-network/ROSAR-framework.

==> tex/05_datasets_exp_results.tex <==
Following the methodology presented in Section \ref{sec:methodology}, this paper aims to propose a framework that improves the robustness of a specific DL object detection model while enhancing its efficiency for embedded detection, such as for an LAUV. 
Before discussing the DL object detection model improvements, we present the models' validation results using the datasets described in \cref{sec:datasets}. 
As an extension of our previous work \cite{aubard2024knowledge}, we utilize the YOLOX model and its transformer extension, YOLOX-ViT. 
Furthermore, since the goal is to leverage the strengths of the knowledge distillation method to improve the performance of lightweight DL models, we compare the results of two YOLOX variants: YOLOX-L, the large model, and YOLOX-Nano, the lighter model. 
While the larger model, YOLOX-L, offers better accuracy, it suffers from lower efficiency and higher power consumption. 
Conversely, the lighter model, YOLOX-Nano, provides higher efficiency but at the cost of reduced accuracy. 
\cref{tab:model-metadata} presents the metadata of these models. 
Despite having approximately the same efficiency when running on the GPU Geforce RTX 3070 Ti (referred to as desktop), the efficiency of YOLOX-L decreases drastically when running on a Jetson TX2 card. % this needs some further explanation why it is like this

\begin{table}
    \caption{YOLOX - Metadata.}
    \label{tab:model-metadata}
    \centering
    \begin{tabular}{l|cccc}
    \toprule
    & L & L-ViT & Nano & Nano-ViT \\
    \midrule
    \# parameters & 54.15M & 50.47M & 0.90M & 0.96M \\
    \midrule
    Gflops per iter. & 155.68 & 152.73 & 1.08 & 1.10 \\
    \midrule
    Desktop Inference time & 0.2913s & 0.3180s & 0.2689s & 0.2802s \\
    Jetson Inference time & 4.52 & 4.55 & 0.56 & 0.57 \\
    \bottomrule
    \end{tabular}
\end{table}

Based on the YOLOX model's specific characteristics, including online data augmentation, raise challenges for performing knowledge distillation (KD). 
Typically, KD requires running the teacher model inference for every student training image; this we call an "online" KD process that can take more than a week of training. 
Due to this limitation, we decided to apply KD "offline", disabling online data augmentation during the student's training, and pre-computing the teacher inference values in advance.
This "offline" method significantly reduces the training time to a few hours.
Given this limitation, we conducted training and validation on six different models: L, L-ViT, Nano, Nano-ViT, Nano-noAug, and Nano-ViT-noAug, where -noAug indicates that online data augmentation is disabled during training. 
Additionally, we trained and compared four more models resulting from KD distillation from the teacher model YOLOX-L to the student model YOLOX-Nano and their transformer versions. 
Specifically:

\begin{itemize}
    \item KD-Nano-noAug-L: KD from L to Nano-noAug
    \item KD-Nano-noAug-L-ViT: KD from L-ViT to Nano-noAug
    \item KD-Nano-ViT-noAug-L: KD from L to Nano-ViT-noAug
    \item KD-Nano-ViT-noAug-L-ViT: KD from L-ViT to Nano-ViT-noAug
\end{itemize}

\cref{tab:dataset-validation} presents the experimental results of the models trained with the SWDD dataset and validated with the three proposed datasets: SWDD-Clean, SWDD-Surface, and SWDD-Noisy. 
The table is organized as follows: \textit{Val.} indicates the validation dataset, \textit{Model} specifies the model used, \textit{$\%$TP} is the percentage of true positive bounding boxes, \textit{FP} is the number of false positive bounding boxes, \textit{Distance} is the average distance between the ground truth middle bounding box and the predicted bounding boxes in pixels, \textit{AP} is the average precision and \textit{$\%$FN} is the percentage of false negative predicted bounding boxes.
As explained in \cref{sec:datasets}, the SSS images have a straight yellow line in the middle representing the nadir gap between the two SSS transducers, which can often be misclassified as a wall. 
To eliminate these incorrect detections, we filtered them from the validation table. 
Round brackets represent this nadir filtering "()" in the \textit{FP} column, where the value inside the brackets indicates the number of false positives removed due to nadir filtering. 
Since the objective of this detection model is to localize the detected targets accurately, the distance from the ground truth bounding box to the predicted bounding box provides valuable insight into which model makes predictions closest to the ground truth.

\begin{table}
\addtolength{\tabcolsep}{-3.975pt}
  \caption{Validation results train with the SWDD and result with the SWDD-Clean, SWDD-Surface, and SWDD-Noisy dataset. In the model names the symbol "*" notes that there was no online data augmentation used.}
  \begin{tabular}{llccccc}
    \toprule
    \textit{Val.} & \textit{Model}         & \textit{$\%$TP} & \textit{FP} & \textit{Distance} & \textit{AP}        & \textit{$\%$FN}       \\
    \midrule
    Clean & L       & 55.2 & 6 (-76)         & \textbf{30.9}            & 0.74 & 45.5        \\
    Clean & L-ViT  & \textbf{62.0} & 10 (-72)  & 36.5   & \textbf{0.76 (+0.24)}           & \textbf{38.3} \\ 
    Clean & Nano        & 52.0 & \textbf{1 (-64)}          & 55.87         & 0.75 (+0.25)          & 48.8       \\
    Clean & Nano-ViT    & 53.2  & 5 (-71)         & 52.11         & 0.74 (+0.26) & 46.7     \\
    \hdashline
    Clean & Nano-*       & 48 & 49          & 56.76         & 0.52          & 52       \\
    Clean & Nano-ViT-*    & 50  & 62         & 52.46         & 0.50 & 49     \\
    \hdashline
    Clean & Nano-*-L       & 79.8 & 65 (-107)          & \textbf{57.9}         & \textbf{0.66 (+0.19)}          & \textbf{25.8}       \\
    Clean & Nano-*-L-ViT    & \textbf{82.2}  & 76 (-148)        & 62.29         & 0.64 (+0.22) & 26.2     \\
    Clean & Nano-ViT-*-L       & \textbf{82.2} & 117 (-108)          & 80.31         & 0.56 (+0.13) & 26.2       \\
    Clean & Nano-ViT-*-L-ViT    & 66.5  & \textbf{64 (-148)}         & 65.7         & 0.59 (+0.23)   & 36.3     \\
    \midrule
    \midrule
    Surface & L       & \textbf{47} & 2 (-0)         & \textbf{31.08}          & \textbf{0.71}  & \textbf{53}        \\
    Surface & L-ViT & 38 & 7  & 41.3   & 0.61           & 62\\
    Surface & Nano       & 7 & 0          & 73.97         & 0.54          & 92       \\
    Surface & Nano-ViT    & 7  & 0          & 38.2         & 0.54      & 92     \\
    \hdashline
    Surface & Nano-*       & 0 & 259          & 0.0         & 0.0          & 100       \\
    Surface & Nano-ViT-*    & 0 & 259          & 0.0         & 0.0         & 100        \\
    \hdashline
    Surface & Nano-*-L       & 52.9 & \textbf{0}          & 68.58         & \textbf{0.75}             & 50.3       \\
    Surface & Nano-*-L-ViT     & \textbf{58.8}  & 28 (-97)        & 85.2         & 0.60 (+0.27)      & \textbf{45.1} \\
    Surface & Nano-ViT-*-L       & 47.7 & 6 (-6)          & 72.64         & 0.68  (+0.05)           & 53.5       \\
    Surface & Nano-ViT-*-L-ViT    & 39.8  & 11 (-27)         & \textbf{53.71}         & 0.59  (+0.16) & 60.1 \\
    \midrule
    \midrule
    Noisy & L        & \textbf{50.0} & 18 (-323)          & 35.8         & \textbf{0.71 (+0.31)}       & \textbf{51.0}     \\
    Noisy & L-ViT & 48.8 & 19 (-120) & \textbf{24.76}   & 0.70 (+0.16)           & 51.3 \\
    Noisy & Nano       & 45.3 & \textbf{1 (-161)} & 29.2         & \textbf{0.71 (+0.22)}          & 54.6 \\
    Noisy & Nano-ViT    & 37.6 & 8 (-208) &  29.3         & 0.67 (+0.24) & 62.3    \\
    \hdashline
    Noisy & Nano-*       & 0.2 & 1298 & 81.2         & 0.0007          & 99 \\
    Noisy & Nano-ViT-*    & 0.2 & 1298 & 81.2         & 0.0007          & 99    \\
    \hdashline
    Noisy & Nano-*-L      & \textbf{74.1} & 247 (-498)          & 48.2         & 0.60 (+0.22)          & 30.0       \\
    Noisy & Nano-*-L-ViT   & 73.5  & \textbf{143 (-542)}        & \textbf{47.0}         & \textbf{0.69 (+0.30)}       & \textbf{28.7}     \\
    Noisy & Nano-ViT-*-L       & 73.5 & 427  (-530)        & 54.8         & 0.49 (+0.17)          & 30.0       \\
    Noisy & Nano-ViT-*-L-ViT    & 64.5  & 218 (-544)         & 45.5         & 0.57 (+0.25)     & 37.2 \\

    \bottomrule
  \end{tabular}
  \label{tab:dataset-validation}
\end{table}

The validation table shows that the L-ViT model provides better results on the SWDD-Clean dataset, which is consistent with the training data. 
However, the L model yields better results on the other two datasets (SWDD-Surface and SWDD-Noisy), which differ from the training data. 
These results suggest that the L model is more robust than its ViT version. 
However, it is essential to note that without filtering the nadir gap, the L model produced significantly more false positives (FP) than its ViT counterpart. 
This indicates that the L model struggles more with distinguishing walls from the nadir. 
Additionally, both the Nano and Nano-ViT versions with data augmentation, despite having fewer FPs, also result in fewer true positives (TP) and a greater distance between the ground truth bounding box and the predicted ones. 
Interestingly, the nano model trained without online data augmentation performs well on the SWDD-Clean dataset, similar to the training data. 
However, its performance significantly drops when validated on datasets with slight noises (SWDD-Surface and SWDD-Noisy). 
The KD versions of these models show improved results, with higher TPs than those trained with online data augmentation. 
However, they also exhibit higher FPs, indicating that these models are less robust. 
The KD-Nano-noAug-L-ViT provides the best overall results among the models without data augmentation.
2
